Option Valuation using Fourier Space Time Stepping

It is well known that the Black-Scholes-Merton model suffers from several deficiencies. Jump-diffusion and Levy models have been widely used to partially alleviate some of the biases inherent in this classical model. Unfortunately, the resulting pricing problem requires solving a more difficult partial-integro differential equation (PIDE) and although several approaches for solving the PIDE have been suggested in the literature, none are entirely satisfactory. All treat the integral and diffusive terms asymmetrically and are difficult to extend to higher dimensions. We present a new, efficient algorithm, based on transform methods, which symmetrically treats the diffusive and integrals terms, is applicable to a wide class of path-dependent options (such as Bermudan, barrier, and shout options) and options on multiple assets, and naturally extends to regime-switching Levy models. We present a concise study of the precision and convergence properties of our algorithm for several classes of options and Levy models and demonstrate that the algorithm is second-order in space and first-order in time for path-dependent options.

==> conclusions.tex <==
\section {Conclusions and Future Work}

We introduced a new method for pricing European and path-dependent options
when the underlying process(es) follows a regime switching L\'evy process(es).
The method treats the integral term and diffusion terms in the pricing PIDE
symmetrically, is efficient, and accurate.

The numerical results attained by the FST method are quite impressive. We
succeeded in reproducing the pricing results obtained by various authors. For
European options, our algorithm is preferable to PIDE finite-difference based
methods since it does not require a time-stepping procedure. Our algorithm is
more appealing than the usual Fourier transform methods since the analytic
expression for the Fourier transform of the option payoff is not required.
Thus, the FST method is the method of choice for European options, especially
with non-standard payoffs. We showed that Barrier options are priced
accurately by comparing with analytical results in the BSM model. Furthermore,
we compare our results for Barrier options under jump models with those of
other authors and find excellent agreement. Additionally, we matched results
obtained by other published methods for American options. This confirms that
the FST is a robust method for pricing options with excellent precision
properties. Moreover, the FST method provides a generic framework for option
pricing under any stock price process, such as Brownian motion, jump-diffusion
or exponential-L\'{e}vy. We also demonstrated how the FST method easily
extends to the multi-dimensional case and can incorporate regime switching.

At this stage of development, the FST algorithm is first order in time. It
should be noted, however, that second order methods in time typically involve
a multi-step or iterative refinement of the solution at each time step. It is
of great interest to investigate various approaches to improve the FST time
order. For American options, this may involve an iterative approach. Barrier
options are more challenging than American options due to the discontinuity in
the option value created by the knock-out / knock-in provisions. In
finite-difference methods, this problem is addressed by refining the mesh
around the point of discontinuity. FFT algorithms, however, are designed for
uniformly spaced points, making mesh refinement difficult to implement.
Fortunately, FFTs using unequal spaced data (NFFT) have been developed
recently. \citeN{potts00_fft_nonequispaced_data} provide an overview of
existing NDFT methods and develop a method of their own. An interesting area
of research would be the use of NFFT algorithms in the FST method to improve
its time-stepping order. Other areas of potential research include:
computation of American exercise boundary, efficient computation of the
Greeks, processes parameter calibration, and stochastic optimal control
problems.

